Synthesize Step-by-Step: Tools, Templates and LLMs as Data Generators for Reasoning-Based Chart VQA

Understanding data visualizations like charts and plots requires reasoning about both visual elements and numerics. Although strong in extractive questions, current chart visual question answering (chart VQA) models suffer on complex reasoning questions. In this work, we address the lack of reasoning ability by data augmentation. We leverage Large Language Models (LLMs), which have shown to have strong reasoning ability, as an automatic data annotator that generates question-answer annotations for chart images. The key innovation in our method lies in the Synthesize Step-by-Step strategy: our LLM-based data generator learns to decompose the complex question into step-by-step sub-questions (rationales), which are then used to derive the final answer using external tools, i.e. Python. This step-wise generation procedure is trained on synthetic data generated using a template-based QA generation pipeline. Experimental results highlight the significance of the proposed step-by-step generation. By training with the LLM-augmented data (LAMENDA), we significantly enhance the chart VQA models, achieving the state-of-the-art accuracy on the ChartQA and PlotQA datasets. In particular, our approach improves the accuracy of the previous state-of-the-art approach from 38% to 54% on the human-written questions in the ChartQA dataset, which needs strong reasoning. We hope our work underscores the potential of synthetic data and encourages further exploration of data augmentation using LLMs for reasoning-heavy tasks.

==> content/01_intro_bhavan.tex <==


\subsection{Bhavan's draft}

% \begin{figure}[h]
% \includegraphics[width=8cm]{media/Chart_VQA_example.png}
% \end{figure}


1) Why is Chart understanding important?
2) What is the issue with current models \cite{liu2022matcha} and the training
3) What is the issue with current datasets
4) Mention LLMs are like human annotators
5) Just like for humans annotators we need to break the task down into simpler tasks by using rationales
6) Just human annotators we do quality check with another LLM


Our contributions:
1) We show the importance of haveing rationales/ step by step breakdown
2)




Visual question answering (VQA) on infographics images which contain charts and plots requires visually understanding the different attributes in the charts and do reasoning on top of it. For example, to answer the question “what is the average of the two lower bars”, the model needs to 
identify different bars and their values, then find the two lower bars and then compute the average of the values. This is a complex task for computer vision models compared to models as it needs models which are good at understadning the visual attributes, reading the text and doing reasoning on top of it.

A lot of the models like MatCha etc, focus heavily on pre-training/fine-tuning using data/tasks which doesn't neccessarily help

We observe a lot of human annotated datasets for chart understading come with a limited number

Large language models (LLMs) and Vision Langauge Models (VLMs) have shown human level intelligence. 

A lot of existing Chart Visual Question Answering datasets 

It's not easy to get annotated real datasets for chart understanding.

Just like training/teaching human annotators with clear broken down steps, we show the importance of teaching a LLM or a VLM




With diagnostic analysis, we show that current SoTA models struggle in reasoning for math and visual information. We aim to address the problem from the perspective of synthetic data. The key idea is that complex reasoning can be decomposed into simpler ones. We explored three methods for synthetic question-answer generation. In the first method, we generate synthetic compositional question-answer pairs using program-based templates. Experiments show that the synthetic questions can bring large performance boost. We train a vision-language model (VLM) which generates data in a more generalizable manner. The final goal is to build an automatic data augmentor, which takes the existing annotated data as input, and generates more complex questions with answers that can be used as training data. 



Charts contain a lot of information and understanding Chart is of utmost importance

Charts contain lot more visual information and to have a model which truely understand

Traditionally we use humans to come up with questions and answers

LLMs are very powerful and so the question, can we use LLMs to augment human annotator?

We want to use original annotated samples and train a VLM to learn to generate the data by learning what the human annotated data looks like

Asking a VLM to generate complex questions could results in lot of biases and bad quality data
so we need to break down into multiple steps just like the way we would teach humans. A crucial aspect of this is to use rationales to breakdown a question 


Approach is use expert annotators like a AI researcher to seed the VLM and then it generates data own it's own

% Use this example in the paper - https://filelist.yaws.link/mnt/efs/bjasani1/data_store/experiments/ChartQA/llava_generated_data/220909_llava-mpt-deplot-chartqa-trainHsynv3pmptnew-ep5_checkpoint-14000/#6364.png


